Efficient learning of quantum interactions from thermal metastable states

Learning quantum interactions from finite-temperature many-body systems is a central task in emerging quantum platforms. Recently, the problem of learning from lattice quantum Gibbs states has found rigorous, efficient protocols. Nevertheless, exact Gibbs states, as the input premise, are in fact computationally intractable to prepare and may not faithfully represent generic finite-temperature quantum systems. In contrast, a system coupled to a heat bath can be stuck at an approximate stationary state (metastable state) long before it truly equilibrates. Here, we formulate a physically and algorithmically consistent alternative: learning from such metastable states of detailed-balanced master equations (Lindbladians) arising from system-bath interactions. We distill the algorithmic mechanism and structural condition underlying Gibbs-state learning and extend it in full to metastable states, attaining nearly optimal sample and computational complexity (in the system size and the precision). More broadly, we sharpen notions of metastability and develop a unified framework for finite-temperature learning.

==> inputs/equation-reference-tags.tex <==
\makeatletter
\MT@newlabel{eq:adb-eta-star}
\MT@newlabel{{eq:adb-eta-star}}
\MT@newlabel{eq:adb-implies-approximate-commutation}
\MT@newlabel{{eq:adb-implies-approximate-commutation}}
\MT@newlabel{eq:coefficient-interface}
\MT@newlabel{{eq:coefficient-interface}}
\MT@newlabel{eq:dyson-high-frequency-kms-integral}
\MT@newlabel{{eq:dyson-high-frequency-kms-integral}}
\MT@newlabel{eq:dyson-high-frequency-operator-bound}
\MT@newlabel{{eq:dyson-high-frequency-operator-bound}}
\MT@newlabel{eq:dyson-low-frequency-active-factor}
\MT@newlabel{{eq:dyson-low-frequency-active-factor}}
\MT@newlabel{eq:dyson-low-frequency-ordered-bound}
\MT@newlabel{{eq:dyson-low-frequency-ordered-bound}}
\MT@newlabel{eq:dyson-low-frequency-telescoping}
\MT@newlabel{{eq:dyson-low-frequency-telescoping}}
\MT@newlabel{eq:dyson-low-frequency-time-integral}
\MT@newlabel{{eq:dyson-low-frequency-time-integral}}
\MT@newlabel{eq:dyson-low-frequency-trace-to-defect}
\MT@newlabel{{eq:dyson-low-frequency-trace-to-defect}}
\MT@newlabel{eq:dyson-low-frequency-word-bound}
\MT@newlabel{{eq:dyson-low-frequency-word-bound}}
\MT@newlabel{eq:filtered-Hamiltonian-local-sum}
\MT@newlabel{{eq:filtered-Hamiltonian-local-sum}}
\MT@newlabel{eq:filtered-Hamiltonian-scalar}
\MT@newlabel{{eq:filtered-Hamiltonian-scalar}}
\MT@newlabel{eq:good-net-candidate-bound}
\MT@newlabel{{eq:good-net-candidate-bound}}
\MT@newlabel{eq:identification-F}
\MT@newlabel{{eq:identification-F}}
\MT@newlabel{eq:identification-F-cut}
\MT@newlabel{{eq:identification-F-cut}}
\MT@newlabel{eq:imaginary-time-negative-basic}
\MT@newlabel{{eq:imaginary-time-negative-basic}}
\MT@newlabel{eq:imaginary-time-positive-basic}
\MT@newlabel{{eq:imaginary-time-positive-basic}}
\MT@newlabel{eq:intro-uniform-ADB-error}
\MT@newlabel{{eq:intro-uniform-ADB-error}}
\MT@newlabel{eq:linearization-error-term}
\MT@newlabel{{eq:linearization-error-term}}
\MT@newlabel{eq:linearized-I}
\MT@newlabel{{eq:linearized-I}}
\MT@newlabel{eq:measurable-Q}
\MT@newlabel{{eq:measurable-Q}}
\MT@newlabel{eq:metastable-identifiability}
\MT@newlabel{{eq:metastable-identifiability}}
\MT@newlabel{eq:operator-fourier-transform-basic}
\MT@newlabel{{eq:operator-fourier-transform-basic}}
\MT@newlabel{eq:outer-cutoff-trace-bound}
\MT@newlabel{{eq:outer-cutoff-trace-bound}}
\MT@newlabel{eq:relations-triangle}
\MT@newlabel{{eq:relations-triangle}}
\MT@newlabel{eq:rotated}
\MT@newlabel{{eq:rotated}}
\MT@newlabel{eq:spatial-truncation-inside-conjugation}
\MT@newlabel{{eq:spatial-truncation-inside-conjugation}}
\MT@newlabel{eq:spatially-truncated-dyson}
\MT@newlabel{{eq:spatially-truncated-dyson}}
\MT@newlabel{eq:sqrt-state-commutator-bound}
\MT@newlabel{{eq:sqrt-state-commutator-bound}}
\MT@newlabel{eq:summary-identification}
\MT@newlabel{{eq:summary-identification}}
\MT@newlabel{eq:tested-commutator-integral}
\MT@newlabel{{eq:tested-commutator-integral}}
\MT@newlabel{eq:tested-product-family}
\MT@newlabel{{eq:tested-product-family}}
\MT@newlabel{eq:tested-stationarity-budget}
\MT@newlabel{{eq:tested-stationarity-budget}}
\MT@newlabel{eq:thermal-lindbladian-basic}
\MT@newlabel{{eq:thermal-lindbladian-basic}}
\MT@newlabel{eq:transferred-Q}
\MT@newlabel{{eq:transferred-Q}}
\MT@newlabel{eq:weak-commutator-defects}
\MT@newlabel{{eq:weak-commutator-defects}}
\MT@newlabel{eq:weak-commutator-identity}
\MT@newlabel{{eq:weak-commutator-identity}}
\MT@newlabel{eq:weak-cutoff}
\MT@newlabel{{eq:weak-cutoff}}
\MT@newlabel{eq:weak-product}
\MT@newlabel{{eq:weak-product}}
\MT@newlabel{eq:weak-scalar-kernel}
\MT@newlabel{{eq:weak-scalar-kernel}}
\MT@newlabel{eq:weak-small-imaginary-time}
\MT@newlabel{{eq:weak-small-imaginary-time}}
\MT@newlabel{eq:gibbs-identifiability}
\MT@newlabel{{eq:gibbs-identifiability}}
\MT@newlabel{eq:overview-pauli-coefficients}
\MT@newlabel{{eq:overview-pauli-coefficients}}
\MT@newlabel{eq:comm-lb-exact-commutator}
\MT@newlabel{{eq:comm-lb-exact-commutator}}
\MT@newlabel{eq:adb-to-local-metastability}
\MT@newlabel{{eq:adb-to-local-metastability}}
\MT@newlabel{eq:thermal-coherent-correction}
\MT@newlabel{{eq:thermal-coherent-correction}}
\MT@newlabel{eq:intro-identifiability}
\MT@newlabel{{eq:intro-identifiability}}
\MT@newlabel{eq:intro-classical-adb}
\MT@newlabel{{eq:intro-classical-adb}}
\MT@newlabel{eq:intro-adb-deviation}
\MT@newlabel{{eq:intro-adb-deviation}}
\MT@newlabel{eq:intro-thermal-dynamics}
\MT@newlabel{{eq:intro-thermal-dynamics}}
\MT@newlabel{eq:adb3-difference-parseval}
\MT@newlabel{{eq:adb3-difference-parseval}}
\makeatother

